2:1 Harmonics in the Radio Light Curves of Supermassive Black Hole Binary Candidates

We present evidence of 2:1 harmonic periodicities in two supermassive black hole binary (SMBHB) candidates (PKS J0805-0111 and PKS 2131-021) in the Owens Valley Radio Observatory (OVRO) + University of Michigan Radio Astronomical Observatory (UMRAO) monitoring programs. This potential discovery follows the previous detection of a 2:1 harmonic periodicity in the SMBHB candidate J1309+1154 from these programs. If confirmed, these suggest a physical origin of blazars exhibiting strong periodicities favoring 2:1 commensurabilities in their light curves. There are significant differences between the 2:1 harmonics in these three blazars, which may be due to differences in their central engines. These three SMBHB candidates demonstrate the importance of careful dissection, i.e. cutting apart and close examination, of blazar light curves, to reveal underlying evidence of coherence between different aspects of the periodicities observed in blazars in the presence of correlated random noise variations. This is particularly important for blazar SMBHB searches, given that the observed periods thus far are all longer than 2 years, and can disappear for long timespans. Harmonics may therefore be crucial in confirming the reality of periodicities and identifying blazar SMBHB candidates. We discuss four models that can account for 2:1 commensurable periodicities in blazar light curves and explain how future detections of shorter period SMBHB candidates, or the lack thereof, may be used to discriminate among the models. Arguments for and against the reality of these periodicities are presented.

==> macros.tex <==
% MACROS.TEX contains generally useful macros, but not those specifically 
%            useful for paper formats.
%
\newcount\figureno  \newcount\tableno
\figureno=0         \tableno=0
%
\newbox\tablebox    \newdimen\tablewidth
%
\newbox\marginbox
\def\strutdepth{\dp\strutbox}
\def\strutheight{\ht\strutbox}
%
\def\smallformat{\hsize=5.5truein\hoffset=0.5truein
    \vsize=8truein\voffset=0.5truein\parskip=1pt}
\def\largeformat{\hsize=6.5truein\hoffset=0.0truein
    \vsize=8.5truein\voffset=0.0truein}
%
\newcount\sectionnumber \newcount\subsectionnumber 
\newcount\subsubsectionnumber
\sectionnumber=0 \subsectionnumber=0 \subsubsectionnumber=0
%
\def\secno{\ifcase\sectionnumber\or
     I\or II\or III\or IV\or V\or VI\or VII\or VIII\or IX\or
     X\or XI\or XII\fi}
\def\subsecno{\ifcase\subsectionnumber\or
     a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or k\or l\fi}
\def\subsubsecno{\ifcase\subsubsectionnumber\or
     i\or ii\or iii\or iv\or v\or vi\or vii\or viii\or ix\or x\fi}
%
\def\section#1\par{\advance\sectionnumber by 1 \subsectionnumber=0
    \vskip 14pt plus 3pt minus 3pt\goodbreak
    \centerline{{\sc\secno.\ #1}}\nobreak\medskip}
\def\subsection#1\par{\advance\subsectionnumber by 1 \subsubsectionnumber=0
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\it\subsecno\/})\ {\it #1}}\nobreak\medskip}
\def\subsubsection#1\par{\advance\subsubsectionnumber by 1
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\eightrm\subsubsecno)}\ {\it #1}}\nobreak\medskip}
%
\def\today{\ifcase\month\or
    January\or February\or March\or April\or May\or June\or
    July\or August\or September\or October\or November\or December\fi
    \space\number\day, \number\year}
%
\def\sol{\ifmmode _{\mathord\odot}
         \else $_{\mathord\odot}$\fi}
\def\deg{\ifmmode ^{\circ}
         \else $^{\circ}$\fi}
\def\pdeg{\ifmmode $\setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}
          \else \setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}$\fi}
% Tony's definitions
\def\vs6{{\vskip 6pt \noindent}}
\def\vs15{{\vskip 15pt \noindent}}
%
\def\arcs{\ifmmode {^{\scriptscriptstyle\prime\prime}}
          \else $^{\scriptscriptstyle\prime\prime}$\fi}
\def\arcm{\ifmmode {^{\scriptscriptstyle\prime}}
          \else $^{\scriptscriptstyle\prime}$\fi}
\newdimen\sa  \newdimen\sb
\def\parcs{\sa=.07em \sb=.03em
     \ifmmode $\rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa$
     \else \rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa\fi}
\def\parcm{\sa=.08em \sb=.03em
     \ifmmode $\rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb$
     \else \rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb\fi}
%
\def\s#1{{\sc #1}}
\def\et{\hbox{\it et al.}}
\def\ET{{\it ET AL.}}
\def\expo#1{\ifmmode \times 10^{#1}
            \else $\times 10^{#1}$\fi}
\def\page{\vfill\eject}
\def\leaderfil{\leaders\hbox to 5pt{\hss.\hss}\hfil}
%
\def\mo{\ifmmode ^{-1}
        \else $^{-1}$\fi}
\def\sup#1{$^{\rm #1}$}
\def\mag{\sup{m}}
\def\muK{\,$\mu$\hbox{K}}
\def\,{\thinspace}
\def\tc#1{3C\,#1}
\def\dots{\relax\ifmmode \ldots
          \else $\ldots$\fi}
\def\WHzsr{\ifmmode $W\,Hz\mo\,sr\mo$
           \else W\,Hz\mo\,sr\mo \fi}
\def\mKs{\ifmmode $\,mK\,s$^{-1/2} 
         \else \,mK\,s$^{-1/2}$ \fi}
\def\microns{\ifmmode \,\mu$m$
             \else \,$\mu$m\fi}
\def\micron{\microns}

%
\def\gsim{\lower.6ex\hbox{$\buildrel>\over\sim$}}
\def\lsim{\lower.6ex\hbox{$\buildrel<\over\sim$}}
\def\ra[#1 #2 #3.#4]{#1\sup{h}#2\sup{m}#3\sup{s}\llap.#4}
\def\dec[#1 #2 #3.#4]{#1\deg#2\arcm#3\arcs\llap.#4}
\def\deco[#1 #2 #3]{#1\deg#2\arcm#3\arcs}
%
\def\refindent{\hangindent=1em \hangafter=1 \noindent}
\def\ref #1;#2;#3;#4\par{\refindent #1,{\it #2},{\bf #3},#4.\par}
\def\ajref #1;#2;#3;#4\par{\refindent #1. #2 {\bf #3},#4.\par}
\def\vref #1\par{\refindent #1.\par}
\def\cref #1;#2;#3;#4;#5\par{\refindent #1, in{\it #2}, 
                             \hbox{ed.}#3 #4, \hbox{p.} #5.\par} 
\def\bref #1;#2;#3\par{\refindent #1, {\it #2} (#3).\par}
%
%
\def\tabl #1\par{\centerline{TABLE \number\tableno}
                 \vskip 7pt
                 \centerline{#1}\nointerlineskip\noindent}
\def\endtable{\tablewidth=\wd\tablebox 
    $$\hss\copy\tablebox\hss$$
    \vskip-\lastskip\vskip -2pt}
\def\tablenote#1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=\parindent \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotenoindent #1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=0pt \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotes #1\par{
            \iftform \goodbreak\topinsert{
                 \centerline{NOTES TO TABLE \number\tableno}
                 \vskip .3cm\noindent
                 \eightpoint\input #1 }\endinsert
            \else \iftabsopen\relax
                  \else\immediate\openout\tabs=junk1\tabsopentrue\fi
                \vskip .5cm
                \centerline{NOTES TO TABLE \number\tableno} \vskip .5cm
                \immediate\write\tabs{\string\etable\space#1\string\par}
            \fi}
\def\doubleline{\vskip 3pt\hrule \vskip 1.5pt \hrule \vskip 5pt}
%
% macros for marginal stuff
%
\def\marginstuff#1{\setbox\marginbox=\vtop{
    \hsize=60pt\tolerance=10000\hbadness=10000
%    \hsize=70pt\tolerance=10000\hbadness=10000
    \parindent=0pt\eightpoint#1\par}\strut}
\def\setmarginal{\strut\vadjust{\kern-\strutdepth\kern-\ht\marginbox\vtop{%
    \moveleft 70pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%    \moveleft 80pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%
% macro for absolute positioning on a page
%
\newdimen\offset 
\newdimen\unita \newdimen\unitb
\newdimen\mina  \newdimen\minb 
%
\unita=1.0cm \mina=0.0cm
\unitb=1.0in \minb=0.0in
%
%
\def\point #1 #2 #3;{\offset=#1\unitb\advance\offset by \minb%
    \rlap{\lower\offset\hbox{\hglue #2\unitb #3}}}%
%
% macros for memos
%
\font\ssq=cmssq8 at 7pt \font\ssbx=cmssbx10 at 12pt 
\setbox0=\hbox{\ssq ATENDEES \rm\quad}
\newdimen\atndwd \atndwd=\wd0
\def\file{}
\def\memo{\hsize=5.875in \hoffset=0.3125in
    \vsize=9in     \voffset=0in
    \elevenpoint
    \vglue -0.8in
    \line{\ssq\hfil INTEROFFICE MEMORANDUM\hfil \llap{\twelvepoint\bf\file}}
    \vskip 10pt
    \centerline{\hbox to 5.4in{\ssbx C A L I F O R N I A\hskip 12pt
                I N S T I T U T E\hskip 12pt O F\hskip 12pt 
                T E C H N O L O G Y}}
    \vskip 30pt}
\def\to#1{\line{\ssq TO \rm\quad #1\hfil\today}
          \vskip 12pt}
\def\from#1{\line{\ssq FROM \rm\quad C. R. Lawrence#1\hfil
                  \ssq EXTENSION \rm\quad 4976\quad\quad
                  \ssq MAIL CODE \rm\quad 105-24}
            \vskip 12pt}
\def\subject#1{\line{\ssq SUBJECT \rm\quad#1\hfil}
               \vskip 12pt}
\def\attendees#1{\hangindent=\atndwd \hangafter=1 \noindent
                \ssq ATENDEES \rm\quad#1
                \vskip 24pt}
\def\OVRO#1{\def\file{OVRO 5m \rlap{#1-87}}}

